Fair Feature Subset Selection using Multiobjective Genetic Algorithm

The feature subset selection problem aims at selecting the relevant subset of features to improve the performance of a Machine Learning (ML) algorithm on training data. Some features in data can be inherently noisy, costly to compute, improperly scaled, or correlated to other features, and they can adversely affect the accuracy, cost, and complexity of the induced algorithm. The goal of traditional feature selection approaches has been to remove such irrelevant features. In recent years ML is making a noticeable impact on the decision-making processes of our everyday lives. We want to ensure that these decisions do not reflect biased behavior towards certain groups or individuals based on protected attributes such as age, sex, or race. In this paper, we present a feature subset selection approach that improves both fairness and accuracy objectives and computes Pareto-optimal solutions using the NSGA-II algorithm. We use statistical disparity as a fairness metric and F1-Score as a metric for model performance. Our experiments on the most commonly used fairness benchmark datasets with three different machine learning algorithms show that using the evolutionary algorithm we can effectively explore the trade-off between fairness and accuracy.

==> Evaluation.tex <==
\section{Evaluation}


This section presents an evaluation of our approach. First, we discuss the datasets, the algorithms induced, and the evaluation metrics selected, followed by our experiments and results. 
\subsection{Data-sets}
\label{subsec:data_acquisition}
%adult data
%german credit score
To evaluate our framework, we used two benchmark datasets: Adult census income, and German Credit Data

\textbf{Adult Census Data: }It includes information for 48,842 different adults across 14 different features. Features include 8 categorical and 6 numerical features. The class label represents whether a person earns more than 50 thousand per year or not, "<=50K" and ">50K" are the values of the class label. The dataset is publicly available and can be accessed from the University of California Irvine (UCI) Machine Learning Repository \footnote{\url{https://archive.ics.uci.edu/ml/datasets/adult}}. 
 
\textbf{German Credit Data: }it consist of the information regarding the 1000 individuals with 20 categorical attributes. Here, each row/data entry represents the person who took a loan from a bank. Each individual is classified as high or low credit risk based on the available set of attributes. Here, 1 represents `Good' credit score, and 2 represents `Bad' credit score. The dataset is also publicly available and can be accessed from the UCI ML Repository \footnote{\url{https://archive.ics.uci.edu/ml/datasets/statlog+(german+credit+data)}}

\textbf{Data Pre-processing: }Machine learning algorithms cannot accept categorical variables unless they are converted into numerical values. It is one of the key steps in data pre-processing. We encode the categorical features of our dataset using label encoding. Label encoding converts each unique categorical value/category to a unique number w.r.t to each column. We used Scikit-Learn \footnote{\url{https://scikit-learn.org/stable/}}, a popular machine learning framework to encode the categorical variable using the label encoder.

% \subsection{Machine learning models used in experiment}
% We trained three different kinds of machine learning models using classification algorithms:
% \begin{itemize}

%     \item \textit{Logistic Regression}~\cite{wright1995logistic} is a statistical supervised learning classification algorithm. A logistic regression-based algorithm, in its pure form, is the function of the independent variable X and results in the probability of a positive outcome i.e. \texttt{P(Y=1)} and is thus extensively used in binary classification problems.

% %Logistic Regression \cite{wright1995logistic} is a supervised learning classification algorithm used to predict the probability of a target variable. The nature of the target or dependent variable is dichotomous, which means there would be only two possible classes.

% %In simple words, the dependent variable is binary in nature having data coded as either 1 (stands for success/yes) or 0 (stands for failure/no).

% %Mathematically, a logistic regression model predicts P(Y=1) as a function of X. It is one of the simplest ML algorithms that can be used for various classification problems such as spam detection, Diabetes prediction, cancer detection



% \item \textit{Support Vector Machines (SVM)}~\cite{suthaharan2016support}
% is a set of supervised learning algorithms with the objective of distinctively separating data points by finding hyperplanes that maximize margins between the data points. This property of SVMs enables its suitability for binary as well as multi-class classification problems.
% %Support vector machines (SVMs) are a set of supervised learning methods used for classification, regression, and outliers detection. The main objective of the support vector machine algorithm is to find a hyperplane in N-dimensional space(N — the number of features) that distinctly classifies the data points. To separate the two classes of data points, there are many possible hyperplanes that could be chosen. Our objective is to find a plane that has the maximum margin, i.e the maximum distance between data points of both classes. Maximizing the margin distance provides some reinforcement so that future data points can be classified with more confidence.


% \item \textit{XGboost~\cite{chen2016xgboost}} is a highly scalable and distributed framework based on gradient boosted decision trees. By efficiently using computing resources, XGboost enables parallelism in decision tree construction thus able to process billions of examples in a short amount of time~\cite{chen2016xgboost}.
% %It is a highly flexible and efficient framework that implements gradient boosted trees. It is quite popular because of its implementation features which include: parallelization of tree construction and continued training. It has been used to solve many data science problems in an accurate manner. XGboost's approach allows both regression and predictive modeling. The main two reasons why it is used is because of its Execution speed and model performance.

% \end{itemize}

 

\subsection{Evaluation Metrics}
We evaluated the performance of machine learning algorithms using the following evaluation metrics.

\begin{itemize}

    \item \textbf{Accuracy: } is the defacto evaluation metrics of machine learning. Accuracy is defined as the fraction of predictions our model got right. It works well when we use an equal number of samples belonging to each class.
    
    \begin{align}
    Accuracy=\frac{TP+TN}{TP+TN+FP+FN}
    \end{align}
    
    \item \textbf{F1-score} is defined as the harmonic mean of precision and recall. Here, Precision evaluates how precise a model is in predicting positive labels. And Recall evaluates the number of correct positive predictions made out of all positive predictions. F1-score ranges between 0 and 1, where 1 is the best and 0 is the worst.
    \begin{align}
        F1-Score = \frac{2*Precision*Recall}{Precision+Recall}
    \end{align}
    
    \begin{align}
            = \frac{2*TP}{2*TP+FP+FN}
    \end{align}

    \item \textbf{Statistical Parity Difference} is defined as the difference between the largest and the smallest group-level selection rate across all values of the sensitive feature(s). Here, the selection rate is defined as the percentage of samples with label 1 (in binary classification). The demographic parity difference of 0 means that all groups have the same selection rate.
      \begin{equation}
            P(\hat{y} =m \mid G=m ) = P( \hat{y}=m \mid G=f ) 
      \end{equation}
    Here, \^ y denotes the decision generated by the model. G is a single protected attribute (race, sex, age, etc.). In this case, our attribute is gender where it can take the value of male or female as per given in the data-sets.
\end{itemize}


